RedAgent: Red Teaming Large Language Models with Context-aware Autonomous Language Agent

Recently, advanced Large Language Models (LLMs) such as GPT-4 have been integrated into many real-world applications like Code Copilot. These applications have significantly expanded the attack surface of LLMs, exposing them to a variety of threats. Among them, jailbreak attacks that induce toxic responses through jailbreak prompts have raised critical safety concerns. To identify these threats, a growing number of red teaming approaches simulate potential adversarial scenarios by crafting jailbreak prompts to test the target LLM. However, existing red teaming methods do not consider the unique vulnerabilities of LLM in different scenarios, making it difficult to adjust the jailbreak prompts to find context-specific vulnerabilities. Meanwhile, these methods are limited to refining jailbreak templates using a few mutation operations, lacking the automation and scalability to adapt to different scenarios. To enable context-aware and efficient red teaming, we abstract and model existing attacks into a coherent concept called "jailbreak strategy" and propose a multi-agent LLM system named RedAgent that leverages these strategies to generate context-aware jailbreak prompts. By self-reflecting on contextual feedback in an additional memory buffer, RedAgent continuously learns how to leverage these strategies to achieve effective jailbreaks in specific contexts. Extensive experiments demonstrate that our system can jailbreak most black-box LLMs in just five queries, improving the efficiency of existing red teaming methods by two times. Additionally, RedAgent can jailbreak customized LLM applications more efficiently. By generating context-aware jailbreak prompts towards applications on GPTs, we discover 60 severe vulnerabilities of these real-world applications with only two queries per vulnerability. We have reported all found issues and communicated with OpenAI and Meta for bug fixes.

==> added.tex <==
% Title
% RedAgent: Leveraging LLM-powered Agent to Jailbreak Large Language Models
% RedAgent: Unleashing the potential of Language Agent in Jailbreaking Large Language Models
% RedAgent: Jailbreaking Large Language Models with Language Agent
% Adaptive Jailbreaking from 
% Improving the Efficiency of Model Red Team with xx 
% Jailbreaking Any 



% Context-aware Fuzzing of Large Language Models via (xx system)
% Context-aware Jailbreak Attacks of Large Language Models via (xx action)
% Leveraging Context Information of Large Language Models to Generate Effectively Context-aware Jailbreak Prompts?
% Context-aware Agentic Red Team in Evaluating Jailbreak Threats of Large Language Models
% 
% The intro sentence of each section
% Method stages rename

\section{Introduction}
% Background of responsible LLMs and their application
The advent of Large Language Models (LLMs) such as GPT-4~\cite{openai2023gpt4} and Gemini~\cite{google2023gemini} represents a significant shift in modern artificial intelligence. 
These models, trained on extensive language corpora sourced from the public domain~\cite{cai2023toolmakers}, excel in a variety of tasks such as natural language processing~\cite{cai2023toolmakers}, code generation~\cite{cai2023toolmakers} and tool using~\cite{cai2023toolmakers}.
Due to their impressive capabilities, LLMs have become integral to specific applications such as GPTs~\cite{cai2023toolmakers}. 
These LLM-integrated applications leverage domain-specific knowledge to enhance their functionality and adaptability to specialized tasks. 
% Prompt-level threats, 引用新闻
As the interaction between LLM and real-world contexts expands, prompt-level security risks have emerged to elicit undesired outputs, including toxic content~(i.e., jailbreak attacks), sensitive information~(i.e., data extraction attacks), and illegal content~(i.e., prompt injection attacks). 
Among these, jailbreak attacks, which use crafted prompts to bypass LLM safeguards and elicit harmful responses, are recognized as the top threat by OWASP, garnering significant attention due to their low cost and severe impact to their application. 
For instance, jailbreak attacks could potentially result in medical assistants giving incorrect and harmful medical advice, shown in Figure x.
% Figure of the harmful content generation in specific application

% Safety alignment
In response to these safety concerns, major LLM developers such as Google DeepMind[], Anthropic[], OpenAI[], and Microsoft[] are dedicated to implementing safety compliance policies and implementing diverse strategies such as RLHF[] in their models. 
Despite these extensive efforts, the generation of harmful content elicited by jailbreak prompts remains a pressing challenge, as evidenced by tens of thousands of effective jailbreak prompts in the wild[].
Therefore, effectively identifying jailbreak vulnerabilities in LLMs is crucial for both their development and real-world deployment, enabling the application of targeted defenses before safety issues occur.



To identify the jailbreak vulnerabilities of LLMs, developing red team methods has become a mainstream approach, focusing on creating jailbreak prompts to simulate potential adversarial scenarios in a black-box setting. 
Typically, given a malicious seed as the goal of the jailbreak (e.g., generate violent content in a video script), a red team first requires human effort to craft specific jailbreak templates, such as the early well-known 'DAN,' through prompt engineering. 
They then leverage the natural language processing capabilities of LLMs to mutate these human-crafted templates (e.g., syntax transformation and synonym replacement) to obtain jailbreak prompts to query the target LLM. Furthermore, they iteratively refine the jailbreak prompts based on the response of the target LLM to enhance their effectiveness, as illustrated in Figure 2.
However, existing red team methods have the following limitations: 
% fail to effectively generate diverse jailbreak prompts due to limitations in four aspects:
% Is it overclaim?
1) Inefficient: The effectiveness of generated jailbreak prompts heavily depend on the initial human-crafted template. This reliance can cause iterative refinement to fail regardless of the number of refinements if the initial template is ineffective.
Additionally, the iterative refinement of jailbreak prompts often fails to obtain useful information if the LLM rejects them, which can be inefficient (e.g., mutating hundreds of times) and impractical in red teaming real-world LLM applications, considering that most of them incorporate rate limits (e.g., 40 messages every 3 hours in GPTs). Further, they cannot effectively seduce novel understanding from the past attacks.
% diversity
2) Lack of diversity: The mutation rules adopted by red team are inherently static~[GPTfuzzer], confining the diversity of the generating novel jailbreak prompts. 
% relevant
3) Irrelevance jailbreaking: They are not well-designed to identify the most relevant risks in specific LLM applications because the malicious seeds are not crafted according to the context. For example, when red teaming code assistants such as Copilot[], it is crucial to focus on automatically identifying potential vulnerabilities that could lead to the generation of unsafe code such as malware[], given that they are proficient in code-related tasks and primarily provide code-related services, rather than expecting them to produce violent or discriminatory content.
% when red teaming healthcare chatbots, it is crucial to focus on automatically identifying potential leaks of sensitive information, such as patient data, rather than expecting the chatbots to generate malware. 
% without explicitly reasoning on the jailbreak prompts 
% cannot effectively learn form experience
% How to reasoning on vulnerabilities
% fail to effectively use context feedback or lack the complex reasoning processes based on insights from previous attacks.
% 
% Challenge, design: 1. effective feedback 2. effective learning

% Guided by the shortcomings of privacy-preserving solutions within the LLM domain, we summarize three key challenges relevant to the development of a privacy-preserving framework for tool-using LLM agents (refer to Figure~\ref{fig:intro}): 
% First, how to achieve a high level of generality in the framework. This includes ensuring that the framework is not limited to specific types of LLMs and tools, whether they are open-source or closed-source.
% Second, how to ensure privacy guarantees within the framework, aligning with existing privacy requirements. 
% Third, how to enable the framework to be adaptable and agnostic to a spectrum of tasks, free from the constraints of specific tasks.
% in later, we should prove that 
Guided by these shortcomings, we summarize the key challenges relevant to building red team methods to efficiently generate diverse jailbreak prompts:
First, how to automatically generate novel jailbreak prompts from a few human-crafted jailbreak templates?
Second, how to draw useful feedback from rejection responses that contain limited information to iteratively refine jailbreak prompts, while ensuring the prompts are relevant to the application scope of the target LLM?
Third, how to effectively learn from past attacks to continuously update the understanding of effective jailbreaks and improve efficiency without much efforts?


In this paper, we introduce a novel model red team method named RedAgent to address these challenges based on the observation 
that LLMs inherently possess the ability to learn and create effective jailbreak prompts from past trials and can understand the intrinstic 
leverage context information
which can naturally ... agent manner. 

% To verify xxx context-aware capability xxx, we jailbreak 60 GPTs using our system and find severe vulnerabilities of GPTs. By comparing the jailbreak attack results on LLM for general use and GPTs, we find 
Furthermore, by , we can red teaming specific LLM applications by the way. To verify this, we jailbreak 60 LLM applications in GPT marketplace.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/system_model.pdf}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}



\section{Background \& Problem Statement}
% This section first outlines typical face recognition systems and illustrates their susceptibility to privacy attacks. Subsequently, considering the weak capabilities of the attackers set in previous privacy-preserving works, we expound upon a more powerful and practical threat model applicable to nearly all face recognition systems, aiming to provide a more realistic assessment of the privacy-preserving capacities.
This section first introduces the definition of LLM and the jailbreak threats of them. Subsequently, we illustrate the system model of typical red team methods towards identifying jailbreak threats of LLMs. We then xxx agent.


\subsection{LLM Jailbreak}
% A basic intro of LLM
A Large Language Model (LLM) is an advanced type of artificial intelligence that processes and generates human-like text based on the patterns and information it has learned from vast amounts of data.[snowflake] LLMs use transformers, a deep learning technique, to understand relationships between all words in a sentence in a self-autoregressive manner as formulated in xx, regardless of their order, which allows LLMs to generate coherent, contextually appropriate text. 
% Symbolic Expression
LLMs exhibit advanced expressive and learning abilities, benefiting from their extensive model sizes, such as GPT-3 with 175 billion and BERT with 340 million. These LLMs have enabled a wide range of real-world applications across various domains, including chatbots (e.g., ChatGPT), writing assistants (e.g., LanguageTool), and advanced search engines (e.g., New Bing3). 

% Main component of LLM
\textbf{Models.}

\textbf{Safety Alignment.}

\textbf{Prompts.} In the inference stage of a Large Language Model (LLM), a prompt is the input text provided by the user, which sets the context and specifies the task for the model to address. This helps guide the generation of relevant and coherent outputs. Alongside this user-provided prompt, there is often a system prompt, which acts as a default prefix implicitly added to the user's input. This system prompt comprises pre-configured instructions or parameters encoded within the model during training, which assist the model in better understanding and responding to the user's request. 
% Symbolic Expression

\textbf{Jailbreak.}
% Definition of jailbreak attacks and Recent work about LLM jailbreaks
An "LLM jailbreak" refers to attempts to manipulate LLMs to bypass their built-in safety mechanisms and content filters. By exploiting specific vulnerabilities in the model's responses, a jailbreak aims to elicit unexpected or forbidden outputs, essentially tricking the model into violating its safety alignments. 
% Jailbreak related work
% Recently, ...
% Recently, some attackers, including security researchers, want to explore the security boundary of LLMs [53]. Besides investigating whether the model could output spontaneously toxic content, attackers also want to induce the model to cross the security fence and output malicious information by prompt engineering [2, 8, 43, 47]. Prompt engineering is the process of constructing text that can be comprehended and interpreted by generative AI models. When this approach is employed for malicious purposes, it is commonly referred as jailbreaking. Jailbreak represents a specialized attack which involving the strategic construction of prompt sequences that make LLMs violate their internal safeguards, resulting in the generation of unexpected or harmful content. The common jailbreak methods focus on role-playing and scenario implantation, intending to let LLMs substitute into specific scenarios and output the malicious content [8, 11, 47]. The input and output of these methods are human readable, but the attacks are less efficient. There are also attack methods that transmit input and output in an encrypted manner [48] so as to avoid detection by the security components of the model, but the readability is poor. These researches predominantly concentrate on the efficacy of attacks, following a result-driven research paradigm.





\subsection{Problem Statement}
% state how model red team work
% A figure of system model





\subsection{Threat Model}
\textbf{Target LLM.} 
In this study, we focus on specific applications powered by text-based LLMs, which serve as the targets for adversaries. 
These applications are securely trained, free from poisoning or any other form of malicious tampering. 
They can enhance their capabilities by using additional domain-specific data for fine-tuning or by leveraging external databases for retrieval-augmented generation. 
Additionally, they may utilize online tools or other built-in functionalities~(e.g., calculators), effectively functioning as holistic agents. 

\textbf{Malicious Intents.} 
In this study, we primarily focus on common jailbreak questions that violates jailbreak attacks aimed at eliciting harmful outputs, such as responses that violate the usage policies of mainstream LLM applications such as hateful, harassing, or violent content, as detailed in Appendix A. 


\textbf{Adversary Goal.} Given the malicious intents as the initial seed, the adversary aims to generate jailbreak prompts that probe the system to elicit harmful outputs in line with these malicious intents via web user interfaces, which are implemented with default security mechanisms. 
In our study, we primarily focus on single-round attacks, as the attacker cannot manipulate the ongoing chat context with the target LLM. 





\subsection{Language Agents.}










% framework
% \subsection{Jailbreak Attacks}
\subsection{Human-centered}
% In the early stage, in-the-wild jailbreaks crafted by prompt engineering emerged in [source]
% heuristically design some principles for generating jailbreak attacks
% Static template, cipher, DrAttack, ASCII attack, low resource language, payload, Making Them Ask and Answer (DRA) 
\subsection{Algorithm-centered}
% gradient + manipulation decoding process
\subsection{LLM-centered}
% PAIR, TAP, GPTFuzzer 
% PAP

% v3
\section{Related Work}
In this section, we provide a comprehensive overview of jailbreak attacks, which can be broadly categorized into three main types based on the nature of the attacker: Human-centered, Algorithm-centered, and LLM-centered. 

\textbf{Human-centered} techniques are among the earliest jailbreak methods, emerging shortly after the release of large language models. These approaches heavily rely on human intuition, experience, and creativity to craft jailbreak prompts. Since the advent of ChatGPT, users have shared numerous jailbreak prompts via social media and websites\cite{Metz2023, Futurism2023, Reddit2022, Guzey2023, Switten2022, Zvi2023}, leading to models generating unexpected or offensive responses, such as pornographic content and hate speech. For instance, attackers have heuristically designed various static jailbreak templates\cite{JailbreakChat2024} or translated harmful prompts into low-resource languages\cite{deng2023multilingual, yong2023low} to circumvent alignment filters. More sophisticated methods such as the ASCII attack\cite{jiang2024artprompt}, DrAttack\cite{li2024drattack}, many-shot jailbreaking\cite{anil2024many} and crafting imaginary scenes with various characters (DeepInception)\cite{li2023deepinception} have also shown effectiveness in generating these attacks.

\textbf{Algorithm-centered} techniques employ computational algorithms to discover effective prompts. For example, Zou et al.\cite{zou2023gcg} introduced the Greedy Coordinate Gradient (GCG) algorithm, which optimizes jailbreak suffixes to maximize the likelihood of affirmative responses to malicious queries based on the gradients of the target LLM. Researchers have also developed genetic algorithms\cite{liu2023autodan, lapid2023open} to mutate and select effective prompts. Furthermore, some studies have drawn connections between jailbreak prompt generation and controlled text generation, employing energy functions to guide the attack process, as seen in the COLD-Attack methodology\cite{guo2024cold}.

\textbf{LLM-centered} techniques leverage the capabilities of large language models to generate and refine jailbreak prompts. GPTFuzzer\cite{yu2023gptfuzzer} utilizes a mutating LLM to generate jailbreak prompts based on manually crafted seed templates, effectively automating the process of prompt variation and exploration. The PAIR framework\cite{chao2023pair} employs an attack model to create and iteratively improve jailbreak prompts based on feedback from the target LLM and the evaluator. Building on this, Mehrotra et al.\cite{mehrotra2023tap} developed TAP, which introduces tree-of-thought reasoning and prunes irrelevant and low-scoring prompts, thus reducing the average number of jailbreak queries and improving the overall success rate. Additionally, PAP\cite{zeng2024pap} regard the target LLM as a human-like communicator and using an attack LLM to generate persuasive jailbreak prompts based on descriptions of persuasion techniques.

% In summary, jailbreak attacks have evolved significantly, from the early human-centered prompt engineering techniques to sophisticated algorithm-centered and LLM-centered methods. This evolution highlights the ongoing challenge of securing LLMs against increasingly complex and automated attacks.

% % v2
% \section{Related Work}
% In this section, we provide a comprehensive overview of jailbreak attacks, which can be broadly categorized into three main types based on the nature of the attacker: Human-centered, Algorithm-centered, and LLM-centered. Figure X illustrates concrete examples of different methods.

% \textbf{Human-centered} techniques are among the earliest jailbreak methods, emerging shortly after the release of large language models. These techniques heavily rely on human intuition, experience, and creativity to craft jailbreak prompts. Since the advent of models like ChatGPT, users have shared numerous jailbreak prompts via social media and websites[], leading to models generating unexpected or offensive responses, such as pornographic content and hate speech. For instance, attackers have translated harmful prompts into low-resource languages[] or used sophisticated cipher methods[] to evade alignment filters. Other approaches include manually crafted imaginary scenes with various characters designed to hypnotize the target LLM into generating uncensored output[].

% \textbf{Algorithm-centered} techniques employ computational algorithms to discover effective prompts. For example, Zou et al.[] introduced the Greedy Coordinate Gradient (GCG) algorithm, which optimizes jailbreak suffixes to maximize the likelihood of affirmative responses to malicious queries based on the gradients of the target LLM. Additionally, researchers have developed genetic algorithms to mutate and select effective prompts. Other studies have connected jailbreak prompt generation with controlled text generation, employing energy functions to guide the attack process, as seen in the COLD-Attack methodology[].

% \textbf{LLM-centered} techniques utilize large language models to generate and refine jailbreak prompts. For instance, GPTFuzzer[] uses a mutate model to generate jailbreak templates based on manually crafted seed prompts. The PAIR framework[] employs an attack model to create and improve jailbreak prompts based on feedback from the target LLM and an evaluator. Building on this, Mehrotra et al.[] developed the TAP algorithm, which filters out irrelevant and low-scoring prompts, thus reducing the average number of jailbreak queries and improving the success rate. Additionally, PAP[] regard the target LLM as a human-like communicator, using it to generate jailbreak prompts based on descriptions of persuasion techniques.

% % v1
% \section{Related Work}
% In this section, we comprehensively introduce the jailbreak attacks. The previous jailbreak efforts can be roughly classified into 3 main categories based on the jailbreak attacker: Human-centered, Algorithm-centered, and LLM-centered. Figure X shows concrete examples of different methods.

% \textbf{Human-based} techniques are one of the earliest attack methods that have been studied and widely discussed, which focus on leveraging human intuition, experience, and creativity to craft jailbreak prompts. From the ChatGPT appear, many users shared their designed jailbreak prompts through social media and websites [], which caused the model to generate unexpected or offensive responses, such as pornographic information, hate speech, etc. For example, people may translate harmful prompts into use low resource language[] or use sophisticated cipher method to encrypt them[] so as to subvert alignment. Some attempts also include mannual crafted imaginary scene with various characters to hypnotize the target LLM to generate uncensored output. 

% \textbf{Algorithm-based} techniques utilize algorithms to explore effective prompts. For example, Zou et al.[] developed greedy coordinate gradient (GCG) algorithm to optimize the jailbreak suffix to maximize the probability of the affirmative response to the malicious query based on the gradients of target LLM. And some researchers developed genetic algorithms to mutate and select effective prompts from attempts[]. Besides, some researchers connect jailbreak prompt generation with controlled text generation and develop a series of energy functions to guide the attack process[COLD-Attack].  

% \textbf{LLM-based} techniques leverage LLM to generate and improve jailbreak prompts. GPTFuzzer[] use a mutate model to generate jailbreak templates based on mannually crafted seed jailbreak prompts. PAIR[] use a attack model to generate jailbreak prompt and improve it based on the feedback from target LLM and evaluator. Based on this, Mehrotra et al.[] develop TAP algorithm, which filtered the target irrelevant prompts and the low-scoring prompts, thereby reducing the average number of jailbreak queries and improving the jailbreak success rate. Besides, PAP regard the LLM as human-like communicator and used the attack LLM to generate jailbreak prompts according to the persuasion technology descriptions.
